Quantification of the propagation of rumors on social media

The propagation of a rumor (unverified information) on a social network is subject to several factors mainly related to the content of this information and especially to the behaviors (profiles) of the actors on this network that retransmit. This state of affairs may vary this propagation as the case may be, and this is what we call the depth of the rumor. This project is tackling this problem. From a real case of the spread of a rumor on Twitter, this contribution proposes an academic approach to quantify the depth of a rumor on social networks and this, for use and interpretation, by specialists concerned by the nature of this information and its auditor.

==> Chapitres/ListeDesAbreviations.tex <==
\chapter*{Liste des Abréviations}

==> fancyvrb/Changes <==
--- fancyvrb.sty
2.8  2010/05/14  - fixed several trailing spaces (hv)
                 - changed license to LPPL
2.7a 2008/02/07  - NMM fixed lastline=firstline bug
2.7  2000/03/21  - changed how fancyvrb.cfg included DG/SR 
2.6  1998/07/17  - Three bug corrected, options numberblanklines,
                   label, labelposition and leftline added and few
                   precisions.
v2.5  1998/01/28 - First public release.
v2.0  1994/03/30 - First version personally shown by Timothy
                   \textsc{van Zandt}


==> fancyvrb/Conclusion.tex <==
\chapter*{Conclusion générale}
\markboth{\textit{Conclusion générale}}{}
\addcontentsline{toc}{chapter}{Conclusion générale}

% But :
Dans ce présent travail, nous avons abordé le problème de la quantification de la profondeur de la diffusion d'une rumeur sur les réseaux sociaux. Contrairement aux approches traditionnelles qui se concentrent sur différents types de modèles de diffusion pour comprendre ces phénomènes, nous avons abordé ici le problème d'un autre point de vue, en étudiant la diffusion à partir d'une situation réelle survenant sur le site de micro-blogging \textbf{Twitter}.

\vspace{0.3cm}
% Généralité sur les RS et les Rumeurs :
% Rs:
En effet, les réseaux sociaux sont devenus un véritable \textit{"phénomène"} de société, car ils ont largement modifié la manière dont nous produisons, diffusons et consommons l’information et fait de chacun une source d'information. La rumeur est émise et répétée plus rapidement et plus largement que jamais, en raison de la connectivité des réseaux sociaux, qui ont un impact sur le monde réel. Un faux tweet a un impact négatif sur la communauté ou la famille, déclenche une panique financière et met même à rude épreuve les relations diplomatiques.

\vspace{0.3cm}
% Etapes de travail :
% Chapitre 01 - 02 - 03 :
Dans ce cadre, nous avons entamé ce travail par une prospection des réseaux sociaux et leurs relations avec la propagation des rumeurs. Aussi, un passage par un état de l'art sur ce qu'a été déjà fait dans ce sens, a été bénéfique pour nous. Comme le phénomène de propagation des rumeurs sur les réseaux sociaux est très récent, l'apport académique est aussi très limité, mais nous avons pu exploiter un ensemble de travaux existant sur la modélisation de diffusion d'information généralement et spécialement de la rumeur, que nous avons jugés utiles pour notre contribution, où nous avons proposé une nouvelle étude basée sur la notion de similarité; afin de calculer la probabilité de diffuser un contenu donné, en étudiant l'effet de la similarité utilisateur-utilisateur et contenu-utilisateur sur la propagation de la rumeur basé sur les sujets d'historique de partage de chaque utilisateur, en utilisant différentes métriques de similarités de textes les plus connues (Cosinus, corrélation de Pearson, Jaccard, Levenshtein et Dice).

\vspace{0.3cm}
% Chapitre 04 :
En guise, d'obtenir des résultats fiables, nous avons utilisé des données réelles à partir du réseau social \textbf{Twitter}, en suivant un ensemble de phases.
 
\vspace{0.2cm}
Premièrement, nous avons re-utilisé deux types d'API afin de télécharger les données utilisateurs. Et nous avons pu collecter \textbf{\textit{17083}} utilisateurs avec \textbf{\textit{25242}} liens entre eux. 

\vspace{0.2cm}
Deuxièmement, nous avons appliqué une extraction des sujets des tweets, en utilisant l'\textbf{API MonkeyLearn}.

\vspace{0.2cm}
Puis l'\textbf{API RxNLP} pour calculer la similarité, en utilisant trois métriques (Cosinus, Jaccard et Dice).

\vspace{0.3cm}
% Résultat :
Finalement, Nous avons évalué nos algorithmes en les déroulant sur ces données et les résultats sont très importants. 

\vspace{0.2cm}
Premièrement, nous avons trouvé que la similarité d'utilisateurs avec le contenu diffusé, n'a aucune relation avec la diffusion de l'information (rumeur), avec l'obtention d'un minimum d'erreur de \textbf{\textit{62.86\%}}. 

\vspace{0.2cm}  
Deuxièmement, nous pouvons déduire que la similarité entre les utilisateurs est très importante, pour la diffusion de l'information (rumeur), car les résultats sont très proches aux données réelles avec un minimum d'erreur de \textbf{\textit{13.09\%}}; c.à.d une précision de \textbf{\textit{86.90\%}}, en utilisant la similarité \textbf{Cosinus} qui a donné le meilleur résultat.

\vspace{0.3cm}
% Perspectives :
Enfin, nous considérons que ce travail ouvre également des perspectives intéressantes en termes de modélisation réalistes, tenant compte des comportements individuels et la sémantique du phénomène qui pourraient être en mesure de prédire, pour un utilisateur donné, s’il transmettra une information ou pas.


==> fancyvrb/README <==

              --------------------------------------------------
              |                   `fancyvrb'                   |
              |                  Version 2.6                   |
              |                 July 17, 1998                  |
              |                                                |
	      | Timothy Van Zandt (Princeton University - USA) |
              |              <tvz@Princeton.EDU>               |
              |                                                |
              |     Packaging, documentation and support       |
              |       Denis Girou (CNRS/IDRIS - France)        |
              |            <Denis.Girou@idris.fr>              |
              |        Sebastian Rahtz (Elsevier - GB)         |
              |           <s.rahtz@elsevier.co.uk>             |
              --------------------------------------------------


  The `fancyvrb' package provides very sophisticated facilities for reading
and writing verbatim TeX code. Users can perform common tasks like changing
font family and size, numbering lines, framing code examples, colouring text
and conditionally processing text.

  `fancyvrb' was heavily used in the typesetting of the "LaTeX Graphics
Companion", by Michel Goossens, Sebastian Rahtz and Frank Mittelbach, Addison
Wesley, 1997.

  It was presented March 31, 1998 for EuroTeX'98. The original paper is
available on (courtesy "Cahiers GUTenberg"):
http://www.univ-rennes1.fr/pub/GUTenberg/publicationsPS/28-29-girou.ps.gz
The description part of `fancyvrb' is not up to date (it was the content
of the version 2.5) but the additional paragraph about it usage to the
typesetting of the "LaTeX Graphics Companion" provide in depth informations
on some usages of `fancyvrb' not described elsewhere.

  The "contrib" subdirectory contain the `fvrb-ex' package (from Denis Girou),
built above `fancyvrb', which offer some "example" environments showing both
the code in verbatim mode and the result of it normally formatted.

                                   Warning!
                                   --------

  * Support is provided by Denis Girou and Sebastian Rahtz and not by
Timothy Van Zandt. Do not bother him with questions relative to `fancyvrb'!

  * The standard `color' package must be available, with a correct "color.cfg"
file defining the dvi converter that must be used.

  * If the `changebar' package is available on your platform, the changes
since the preceding version will be marked by special gray bars printed
in the margins. But the driver name must be hardcoded in the file.
So, if you have `changebar' and are not using the "dvips" driver, change this
name in the line
             {\ChangeBartrue\usepackage[dvips,rightbars]{changebar}}{}
in fancyvrb.dtx (the other drivers supported by this package are "dvitoln03",
"dvitops" and "emtex").
    If you really need to desactivate this feature (it must not be the case,
as there will be no effect if you haven't `changebar', and, if you have it,
it must work on your platform...) just change the two relevant lines to:
\IfFileExists{changebar.sty}{}{}

.............................................................................

     Comments, suggestions and bug reports (with version number and the
keyword "fancyvrb" in the subject of the message) to <Denis.Girou@idris.fr>
and <s.rahtz@elsevier.co.uk>


